The Influence of Prior Discourse on Conversational Agent-Driven Decision-Making

Persuasion through conversation has been the focus of much research. Nudging is a popular strategy to influence decision-making in physical and digital settings. However, conversational agents employing "nudging" have not received significant attention. We explore the manifestation of cognitive biases-the underlying psychological mechanisms of nudging-and investigate how the complexity of prior dialogue tasks impacts decision-making facilitated by conversational agents. Our research used a between-group experimental design, involving 756 participants randomly assigned to either a simple or complex task before encountering a decision-making scenario. Three scenarios were adapted from Samuelson's classic experiments on status-quo bias, the underlying mechanism of default nudges. Our results aligned with previous studies in two out of three simple-task scenarios. Increasing task complexity consistently shifted effect-sizes toward our hypothesis, though bias was significant in only one case. These findings inform conversational nudging strategies and highlight inherent biases relevant to behavioural economics.

==> Tables/demographics.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Characteristic} & \textbf{Value} \\ \midrule
N & 756 \\
Age (years) & 41.81 $\pm$ 13.54 (18--81) \\
Time (min) & 10.53 $\pm$ 301.53 (1.48--42.73) \\
Sex & 50.4\% male (381), 49.6\% female (375) \\
Ethnicity & White: 79.6\% (602), Black: 10.2\% (77), \\
          & Mixed: 4.4\% (33), Asian: 4.4\% (33), \\
          & Other: 0.9\% (7), Unavailable: 0.5\% (4) \\
Birth Country & UK: 60.6\% (458), US: 31.5\% (238), Other: 7.9\% (60) \\
Residence & UK: 66.1\% (500), US: 32.9\% (249), Ireland: 0.9\% (7) \\
Nationality & UK: 62.2\% (470), US: 32.2\% (243), Other: 5.6\% (43) \\
Language & English (100\%, 756) \\
Student Status & Not student: 73.5\% (556), Student: 11.1\% (84), \\
               & Missing: 15.3\% (116) \\
Employment Status & Full-time: 42.7\% (323), Part-time: 18.3\% (138), \\
                  & Not in paid work: 12.8\% (97), Unemployed: 5.2\% (39), \\
                  & Unclassified: 2.6\% (20), New job: 0.8\% (6), \\
                  & Missing: 17.6\% (133) \\
\bottomrule
\end{tabular}
\caption{Detailed Demographic and employment characteristics of the sample (N = 756).}
\label{tab:demographics}
\end{table}


==> Tables/new/table_ct_sqneut.tex <==
% \begin{table*}[ht]
%         \centering
%         \resizebox{\columnwidth}{!}{%
%         \renewcommand{\arraystretch}{1.5} % Increases line spacing
%         \label{sec:sqb framing vs non-sqb framing}%
%         \begin{tabular}{lllllllll}%
%           \hline%
%           \multirow{3}{*}{Alternatives}&\multicolumn{3}{c}{Choice rates}&&\multicolumn{4}{c}{Status quo framing vs. neutral framing}\\%
%           \cline{2%
%             -%
%             4}%
%           \cline{6%
%             -%
%             9}%
%                                                                   &   &   &   &   &   &   &   &   \\%
%           &SQ&N&NSQ&&$\chi^2$&\textit{p}&Odds ratio \newline%
%           (95\% CI)&Cohen's h \newline%
%           (95\%CI)\\%
%           \hline%
%           \textbf{Scenario 1: Budget allocation ratios} &   &   &   &   &   &   &   &   \\%
%           60A40H                                                   & 20/37 (0.54) & 9/39 (0.23) & 7/41 (0.17) &  & 7.72& 0.005*& 0.26 [0.1, 0.68]& -0.65 [-1.35, 0.05] \\%
%           50A50H                                                   & 34/41 (0.83) & 30/39 (0.77) & 17/37 (0.46) &  & 0.45& 0.502& 1.46 [0.48, 4.39]& 0.15 [-0.63, 0.93] \\%
%           \textbf{Scenario 2: Investment portfolios}    &   &   &   &   &   &   &   &   \\%
%           Mod. Risk                                                & 33/39 (0.85) & 35/41 (0.85) & 27/36 (0.75) &  & 0.01& 0.925& 1.06 [0.31, 3.62]& 0.02 [-0.85, 0.89] \\%
%           High Risk                                                & 9/36 (0.25) & 6/41 (0.15) & 6/39 (0.15) &  & 1.31& 0.252& 1.94 [0.62, 6.13]& 0.26 [-0.55, 1.07]  \\%
%           \textbf{Scenario 3: College jobs }            &   &   &   &   &   &   &   &   \\%
%           College A                                                & 24/40 (0.6) & 20/39 (0.51) & 19/40 (0.48) &  & 0.61& 0.435& 0.7 [0.29, 1.71]& -0.18 [-0.81, 0.45] \\%
%           College B                                                & 21/40 (0.52) & 19/39 (0.49) & 16/40 (0.4) &  & 0.11& 0.737& 1.16 [0.48, 2.81]& 0.08 [-0.55, 0.7] \\%
%           \hline%
%         \end{tabular}
%         }
%         \newline
%         \caption{Complex Task - Status quo framing vs. neutral framing}
%         \label{tab:CT-SQNEUT}
%       \end{table*}

==> Tables/new/table_st_sqneut.tex <==
% \begin{table*}[ht]
%         \centering
%         \resizebox{\columnwidth}{!}{%
%         \renewcommand{\arraystretch}{1.5} % Increases line spacing
%         \label{sec:sqb framing vs non-sqb framing}%
%         \begin{tabular}{lllllllll}%
%           \hline%
%           \multirow{3}{*}{Alternatives}&\multicolumn{3}{c}{Choice rates}&&\multicolumn{4}{c}{Status quo framing vs. neutral framing}\\%
%           \cline{2%
%             -%
%             4}%
%           \cline{6%
%             -%
%             9}%
%                                                                   &   &   &   &   &   &   &   &   \\%
%           &SQ&N&NSQ&&$\chi^2$&\textit{p}&Odds ratio \newline%
%           (95\% CI)&Cohen's h \newline%
%           (95\%CI)\\%
%           \hline%
%           \textbf{Scenario 1: Budget allocation ratios} &   &   &   &   &   &   &   &   \\%
%           60A40H                                                   & 16/41 (0.39) & 12/42 (0.29) & 4/42 (0.1) &  & 1.01& 0.314& 0.62 [0.25, 1.56]& -0.22 [-0.87, 0.43] \\%
%           50A50H                                                   & 38/42 (0.9) & 30/42 (0.71) & 25/41 (0.61) &  & 4.94& 0.026*& 3.8 [1.11, 12.98]& 0.5 [-0.37, 1.37]  \\%
%           \textbf{Scenario 2: Investment portfolios}    &   &   &   &   &   &   &   &   \\%
%           Mod. Risk                                                & 32/42 (0.76) & 32/40 (0.8) & 33/42 (0.79) &  & 0.17& 0.677& 1.25 [0.44, 3.58]& 0.09 [-0.65, 0.84] \\%
%           High Risk                                                & 9/42 (0.21) & 8/40 (0.2) & 10/42 (0.24) &  & 0.03& 0.873& 1.09 [0.37, 3.18]& 0.04 [-0.72, 0.79]   \\%
%           \textbf{Scenario 3: College jobs }            &   &   &   &   &   &   &   &   \\%
%           College A                                                & 25/41 (0.61) & 19/41 (0.46) & 21/41 (0.51) &  & 1.77& 0.184& 0.55 [0.23, 1.33]& -0.29 [-0.92, 0.33] \\%
%           College B                                                & 20/41 (0.49) & 22/41 (0.54) & 16/41 (0.39) &  & 0.2& 0.659& 0.82 [0.35, 1.96]& -0.1 [-0.71, 0.52]  \\%
%           \hline%
%         \end{tabular}
%         }
%         \newline
%         \caption{Simple Task - Status quo framing vs. neutral framing}
%         \label{tab:ST-SQNEUT}
%       \end{table*}

==> Tables/supp_material/all_decision_scenarios.tex <==

\section{Decision Scenarios}
\label{sec:appendix-ds}
\subsection{Budget Allocation}
\label{sec:appendix-ds-ba}
\subsubsection{Neutral Condition}
\label{sec:appendix-ds-ba-neut1}

\begin{quote}
The National Highway Safety Commission is deciding how to allocate its budget between two safety research programs:
\begin{enumerate}
    \item Improving automobile safety (bumpers, body, gas tank configuration, seat-belts), and
    \item Improving the safety of interstate highways (guard rails, grading, highway interchanges, and implementing selective reduced speed limits).
\end{enumerate}

Since there is a ceiling on its total spending, it must choose between the options provided below. If you had to make this choice, which of the following will you choose?
 \begin{itemize}
     \item Allocate 60\% to auto safety and 40\% to highway safety
     \item Allocate 50\% to auto safety and 50\% to highway safety
 \end{itemize}
\end{quote}

\subsubsection{Neutral Condition - Alternative Swapped}
\label{sec:appendix-ds-ba-neut2}

\begin{quote}

The National Highway Safety Commission is deciding how to allocate its budget between two safety research programs:
\begin{enumerate}
    \item Improving automobile safety (bumpers, body, gas tank configuration, seat-belts), and
    \item Improving the safety of interstate highways (guard rails, grading, highway interchanges, and implementing selective reduced speed limits).
\end{enumerate}

Since there is a ceiling on its total spending, it must choose between the options provided below. If you had to make this choice, which of the following will you choose?
 \begin{itemize}
     \item Allocate 50\% to auto safety and 50\% to highway safety.
     \item Allocate 60\% to auto safety and 40\% to highway safety.
 \end{itemize}


    
\end{quote}

\subsubsection{Status Quo - 60A40H }
\label{sec:appendix-ds-ba-sq60a40h}

\begin{quote}

The National Highway Safety Commission is deciding how to allocate its budget between two safety research programs:
\begin{enumerate}
    \item Improving automobile safety (bumpers, body, gas tank configuration, seat-belts)
    \item Improving the safety of interstate highways (guard rails, grading, highway interchanges, and implementing selective reduced speed limits).
\end{enumerate}

Currently, the commission allocates approximately 60\% of its funds to auto safety and 40\% of its funds to highway safety.
Since there is a ceiling on its total spending, it must choose between the options provided below. If you had to make this choice, which of the following will you choose?
 \begin{itemize}
     \item Maintain present budget amounts for the programs.
     \item Decrease auto program by 10\% and raise highway program by like amount.
 \end{itemize}
    
\end{quote}

\subsubsection{Status Quo - 50A50H }
\label{sec:appendix-ds-ba-sq50a50h}

\begin{quote}

The National Highway Safety Commission is deciding how to allocate its budget between two safety research programs: 
\begin{enumerate}
    \item Improving automobile safety (bumpers, body, gas tank configuration, seat-belts)
    \item Improving the safety of interstate highways (guard rails, grading, highway interchanges, and implementing selective reduced speed limits).
\end{enumerate}

Currently, the commission allocates approximately 50\% of its funds to auto safety and 50\% of its funds to highway safety.
Since there is a ceiling on its total spending, it must choose between the options provided below. If you had to make this choice, which of the following will you choose? 

 \begin{itemize}
     \item Maintain present budget amounts for the programs.
     \item Increase auto program by 10\% and lower highway program by like amount.
 \end{itemize}

\end{quote}

\subsection{Investment Decision Making}
\label{sec:appendix-ds-idm}

\subsubsection{Neutral Condition}
\label{sec:appendix-ds-idm-neut1}

\begin{quote}

You are a serious reader of the financial pages but until recently have had few funds to invest. That is when you inherited a large sum of money from your great uncle. You are considering different portfolios.
Your choices are:
 \begin{itemize}
     \item Invest in moderate-risk Company A. Over a year's time, the stock has .5 chance of increasing 30\% in value, a .2 chance of being unchanged, and a .3 chance of declining 20\% in value.
     \item Invest in high-risk Company B. Over a year's time, the stock has a .4 chance of doubling in value, a .3 chance of being unchanged, and a .3 chance of declining 40\% in value.
 \end{itemize}
    
\end{quote}

\subsubsection{Neutral Condition - Alternative Swapped}
\label{sec:appendix-ds-idm-neut2}

\begin{quote}

You are a serious reader of the financial pages but until recently have had few funds to invest. That is when you inherited a large sum of money from your great uncle. You are considering different portfolios.
Your choices are:
 \begin{itemize}
     \item Invest in high-risk Company B. Over a year's time, the stock has a .4 chance of doubling in value, a .3 chance of being unchanged, and a .3 chance of declining 40\% in value.
     \item Invest in moderate-risk Company A. Over a year's time, the stock has .5 chance of increasing 30\% in value, a .2 chance of being unchanged, and a .3 chance of declining 20\% in value.
 \end{itemize}
 
    
\end{quote}

\subsubsection{Status Quo - Moderate Risk}
\label{sec:appendix-ds-idm-modrisk}

\begin{quote}
    You are a serious reader of the financial pages but until recently have had few funds to invest. That is when you inherited a portfolio of cash and securities from your great uncle. A significant portion of this portfolio is invested in moderate-risk Company A. You are deliberating whether to leave the portfolio intact or change it by investing in other securities. (The tax and broker commission consequences of any change are insignificant.)
Your choices are:
 \begin{itemize}
     \item Retain the investment in moderate-risk Company A. Over a year's time, the stock has .5 chance of increasing 30\% in value, a .2 chance of being unchanged, and a .3 chance of declining 20\% in value.
     \item Invest in high-risk Company B. Over a year's time, the stock has a .4 chance of doubling in value, a .3 chance of being unchanged, and a .3 chance of declining 40\% in value.
 \end{itemize}
\end{quote}

\subsubsection{Status Quo - High Risk}
\label{sec:appendix-ds-idm-highrisk}

\begin{quote}
    You are a serious reader of the financial pages but until recently have had few funds to invest. That is when you inherited a portfolio of cash and securities from your great uncle. A significant portion of this portfolio is invested in high-risk Company B. You are deliberating whether to leave the portfolio intact or change it by investing in other securities. (The tax and broker commission consequences of any change are insignificant.)
Your choices are:
 \begin{itemize}
     \item Retain the investment in high-risk Company B. Over a year's time, the stock has a .4 chance of doubling in value, a .3 chance of being unchanged, and a .3 chance of declining 40\% in value.
     \item Invest in moderate-risk Company A. Over a year's time, the stock has a .5 chance of increasing 30\% in value, a .2 chance of being unchanged, and a .3 chance of declining 20\% in value.
 \end{itemize}
\end{quote}


\subsection{College Jobs}
\label{sec:appendix-ds-cj}

\subsubsection{Neutral Condition}
\label{sec:appendix-ds-cj-neut1}

\begin{quote}
    Having just completed your graduate degree, you have two offers of teaching jobs in hand.
When evaluating teaching job offers, people typically consider the salary, the reputation of the school, the location of the school, and the likelihood of getting tenure (tenure is permanent job contract that can only be terminated for cause or under extraordinary circumstances).
Your choices are:
 \begin{itemize}
     \item College A: east coast, very prestigious school, high salary, fair chance of tenure.
     \item College B: west coast, low prestige school, high salary, good chance of tenure.
 \end{itemize}
\end{quote}

\subsubsection{Neutral Condition - Alternative Swapped}
\label{sec:appendix-ds-cj-neut2}

\begin{quote}
    Having just completed your graduate degree, you have two offers of teaching jobs in hand.
When evaluating teaching job offers, people typically consider the salary, the reputation of the school, the location of the school, and the likelihood of getting tenure (tenure is permanent job contract that can only be terminated for cause or under extraordinary circumstances).
Your choices are:
 \begin{itemize}
     \item College B: west coast, low prestige school, high salary, good chance of tenure.
     \item College A: east coast, very prestigious school, high salary, fair chance of tenure.
 \end{itemize}
\end{quote}

\subsubsection{Status Quo - College A}
\label{sec:appendix-ds-cj-colla}
You are currently an assistant professor at College A in the east coast. Recently, you have been approached by colleague at other university with job opportunity.
When evaluating teaching job offers, people typically consider the salary, the reputation of the school, the location of the school, and the likelihood of getting tenure (tenure is permanent job contract that can only be terminated for cause or under extraordinary circumstances).
Your choices are:
 \begin{itemize}
     \item Remain at College A: east coast, very prestigious school, high salary, fair chance of tenure.
     \item Move to College B: west coast, low prestige school, high salary, good chance of tenure.
 \end{itemize}
\begin{quote}
    
\end{quote}

\subsubsection{Status Quo - College B}
\label{sec:appendix-ds-cj-collb}
You are currently an assistant professor at College B in the west coast. Recently, you have been approached by colleague at other university with job opportunity.
When evaluating teaching job offers, people typically consider the salary, the reputation of the school, the location of the school, and the likelihood of getting tenure (tenure is permanent job contract that can only be terminated for cause or under extraordinary circumstances). 
Your choices are:
 \begin{itemize}
     \item Remain at College B: west coast, low prestige school, high salary, good chance of tenure.
     \item Move to College A: east coast, very prestigious school, high salary, fair chance of tenure.
 \end{itemize}
\begin{quote}
    
\end{quote}


==> Tables/supp_material/complex_task_questions.tex <==
\begin{longtable*}[c]{@{}ccccc@{}}
\toprule
\textbf{Domain} & \multicolumn{3}{c}{\textbf{Attribute}} & \textbf{Questions} \\* \midrule
\endfirsthead
%
\multicolumn{5}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\toprule
\textbf{Domain} & \multicolumn{3}{c}{\textbf{Attribute}} & \textbf{Questions} \\* \midrule
\endhead
%
\bottomrule
\endfoot
%
\endlastfoot
%
\textbf{\begin{tabular}[c]{@{}c@{}}Home \\ Property\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ Bedrooms\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Size \\ (Sq ft.)\end{tabular}} & \textbf{Property Reviews} & \textbf{} \\* \midrule
1st & Three Rooms & 2000 & Four star & \begin{tabular}[c]{@{}c@{}}In the following scenario choose \\ from various property recommendations.\end{tabular} \\
2nd & Two times 1st & Same as first & Same as first & \begin{tabular}[c]{@{}c@{}}The first property has three bedrooms, \\ 2000 square feet, and a 4-star rating. \\ The second property has twice the number of\\  bedrooms and with the same size and rating. \\ Which one do you prefer, and why?\end{tabular} \\
3rd & Same as the second & Half of first & Same as first & \begin{tabular}[c]{@{}c@{}}The third property has the same \\ number of bedrooms as the second one \\ but is half the size of the first one,\\  with the same rating as the first. \\ Which one do you prefer, and why?\end{tabular} \\
4th & Same as the second & Same as third & \begin{tabular}[c]{@{}c@{}}One star less \\ than the first\end{tabular} & \begin{tabular}[c]{@{}c@{}}The fourth property has the same \\ number of bedrooms as the second, \\ the same size as the third, but \\ one less star rating than the first. \\ Which one do you prefer, and why?\end{tabular} \\
 &  &  &  & \begin{tabular}[c]{@{}c@{}}Remember the details \\ of the fourth property. \\ Specific information \\ will be requested later.\end{tabular} \\* \midrule
\textbf{\begin{tabular}[c]{@{}c@{}}Music\\ Artist\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Live \\ Performances\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Artist \\ Remuneration \\ for Show\end{tabular}} & \textbf{Artist-Specific} & \textbf{} \\* \midrule
1st & Three & 2000 Units & Four star & \begin{tabular}[c]{@{}c@{}}In the following scenario choose\\  from various artist recommendations.\end{tabular} \\
2nd & 2 times 1st & Same as first & Same as first & \begin{tabular}[c]{@{}c@{}}The first artist performs\\  three live shows, \\ is paid 2000 units per show, \\ and has a 4-star rating. \\ The second artist performs \\ twice as many shows, \\ with the same pay and rating. \\ Which artist do you prefer, and why?\end{tabular} \\
3rd & Same as the second & Half of first & Same as first & \begin{tabular}[c]{@{}c@{}}he third artist performs the same\\  number of shows as the second, \\ earns half the pay of the first artist, \\ but has the same rating as the first. \\ Which artist do you prefer, and why?\end{tabular} \\
4th & Same as the second & Same as third & \begin{tabular}[c]{@{}c@{}}One star less \\ than the first\end{tabular} & \begin{tabular}[c]{@{}c@{}}The fourth artist performs the \\ same number of shows as the second, \\ earns the same pay as the third, but \\ has two stars less than the first artist. \\ Which artist do you prefer, and why?\end{tabular} \\
 &  &  &  & \begin{tabular}[c]{@{}c@{}}Remember the \\ details of the fourth artist. \\ Specific information\\  will be requested later.\end{tabular} \\* \midrule
\textbf{\begin{tabular}[c]{@{}c@{}}Movies - \\ Streaming \\ Service\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ Parallel Devices\end{tabular}} & \textbf{Library Size} & \textbf{Service Rating} & \textbf{} \\* \midrule
1st & Three & 2000 Movies & Four star & \begin{tabular}[c]{@{}c@{}}In the following scenario choose from \\ various streaming service recommendations.\end{tabular} \\
2nd & 2 times 1st & Same as first & Same as first & \begin{tabular}[c]{@{}c@{}}The first streaming service supports \\ 3 parallel devices, \\ has a library of 2000 movies,\\  and is rated 4 stars. \\ The second service supports \\ twice as many devices, \\ with the same library size and rating. \\ Which service do you prefer, and why?\end{tabular} \\
3rd & Same as the second & Half of first & Same as first & \begin{tabular}[c]{@{}c@{}}The third streaming service supports the\\  same number of devices as the second, has \\ half the library size of the first,\\  but has the same rating as the first. \\ Which service do you prefer, and why?\end{tabular} \\
4th & Same as the second & Same as third & \begin{tabular}[c]{@{}c@{}}One star less\\  than the first\end{tabular} & \begin{tabular}[c]{@{}c@{}}The fourth streaming service supports\\  the same number of devices as the second, \\ has the same library size as the third,\\  but is rated one star less than the first. \\ Which service do you prefer, and why?\end{tabular} \\
 &  &  &  & \begin{tabular}[c]{@{}c@{}}Remember the details of the fourth service. \\ Specific information will be requested later.\end{tabular} \\*
\midrule
\textbf{\begin{tabular}[c]{@{}c@{}}Calendar\\ App\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Calendar Syncing \\ Across Devices\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Managed \\ Tasks \\ Per Year\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Event Privacy \\ Rating\end{tabular}} & \textbf{} \\* 
\midrule
1st & 3 & 2000 & Four star & \begin{tabular}[c]{@{}c@{}}In the following scenario choose from \\ Various Apps recommendations for calendar.\end{tabular} \\
2nd & 2 times 1st & Same as first & Same as first & \begin{tabular}[c]{@{}c@{}}The first calendar app can sync\\  across three devices, \\ manages 2000 tasks per year,\\  and has a 4-star privacy rating. \\ The second app syncs across two devices, \\ manages the same number of tasks,\\  and has the same privacy rating. \\ Which app do you prefer, and why?\end{tabular} \\
3rd & Same as Second & Half of first & Same as first & \begin{tabular}[c]{@{}c@{}}The third app syncs across the same\\  number of devices as the second app, \\ but manages half as\\  many tasks as the first app, \\ with the same privacy rating as the first. \\ Which app do you prefer, and why?\end{tabular} \\
4th & Same as Second & Same as third & \begin{tabular}[c]{@{}c@{}}One star less\\  than the first\end{tabular} & \begin{tabular}[c]{@{}c@{}}The fourth app syncs across the same number \\ of devices as the second, manages the same\\  number of tasks as the third, but has one less \\ star in privacy rating compared to the first. \\ Which app do you prefer, and why?\end{tabular} \\
 &  &  &  & \begin{tabular}[c]{@{}c@{}}Remember the details of the fourth App. \\ Specific information will be requested later.\end{tabular} \\* 
 
 \midrule
\textbf{Bank} & \textbf{\begin{tabular}[c]{@{}c@{}}Bank Branch \\ Proximity\end{tabular}} & \textbf{Interest Rates} & \textbf{\begin{tabular}[c]{@{}c@{}}Fee-Free \\ Accounts\\  Rating\end{tabular}} & \textbf{} \\* 
\midrule
1st & 3km & 2000 units & Four & \begin{tabular}[c]{@{}c@{}}In the following scenario choose \\ from various banks recommendations.\end{tabular} \\
2nd & 2 times 1st & Same as first & Same as first & \begin{tabular}[c]{@{}c@{}}The first bank is 3 km away,\\  offers 2000 units of interest, \\ and has a four-star rating for fee-free accounts. \\ The second bank is twice as far away, \\ offers the same amount of interest,\\  and has the same fee-free account rating. \\ Which bank would you prefer, and why?\end{tabular} \\
3rd & Same as the second & Half of first & Same as first & \begin{tabular}[c]{@{}c@{}}The third bank is as far away as the second bank, \\ offers half the amount of interest as \\ the first bank, but has the same fee-free\\  account rating as the first bank. \\ Which bank would you prefer, and why?\end{tabular} \\
4th & Same as the second & Same as third & \begin{tabular}[c]{@{}c@{}}One star less \\ than the first\end{tabular} & \begin{tabular}[c]{@{}c@{}}The fourth bank is as far\\  away as the second bank, \\ offers the same amount of interest as the third bank, \\ but has one star less in fee-free account rating\\  compared to the first bank. \\ Which bank would you prefer, and why?\end{tabular} \\*

\midrule
\textbf{\begin{tabular}[c]{@{}c@{}}Messaging \\ App\end{tabular}} & 
\textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ Simultaneous \\Devices\end{tabular}} & 
\textbf{\begin{tabular}[c]{@{}c@{}}Messages \\ Per Day\end{tabular}} & 
\textbf{\begin{tabular}[c]{@{}c@{}}Security \\ Rating\end{tabular}} & 
\textbf{} \\* 
\midrule

1st & 3 & 2000 & Four star & 
\begin{tabular}[c]{@{}c@{}}In the following scenario, choose from \\ various messaging app recommendations.\end{tabular} \\ 
2nd & 2 times 1st & Same as first & Same as first & 
\begin{tabular}[c]{@{}c@{}}The first messaging app allows access \\ on three devices, supports 2000 messages per day, \\ and has a 4-star security rating. \\ The second app allows access on\\ twice as many devices, \\ supports the same number of messages, \\ and has the same security rating. \\ Which app do you prefer, and why?\end{tabular} \\ 
3rd & Same as the second & Half of first & Same as first & 
\begin{tabular}[c]{@{}c@{}}The third app allows access on the same \\ number of devices as the second app, \\ but supports half as many messages as the first app, \\ with the same security rating as the first. \\ Which app do you prefer, and why?\end{tabular} \\ 
4th & Same as the second & Same as third & One star less than the first & 
\begin{tabular}[c]{@{}c@{}}The fourth app allows access on the \\ same number of devices as the second, \\ supports the same number \\ of messages as the third, \\ but has one less star in \\security rating compared to the first. \\ Which app do you prefer, and why?\end{tabular} \\ 
& & & & 
\begin{tabular}[c]{@{}c@{}}Remember the details\\ of the fourth app, \\ including the number\\ of devices, messages per day, \\ and its security rating.\\ Specific information \\ will be requested later.\end{tabular} \\* 
% \bottomrule

\caption{Complex Tasks for prior discourse.}
\label{tab:my-table}\\
\end{longtable*}

==> Tables/supp_material/simple_task_questions.tex <==
\begin{table*}[ht]
\centering
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{lll}
\hline
\textbf{Domain}                    & \textbf{Attribute}           & \textbf{Yes/No Questions}                                                          \\ \hline
\multirow{6}{*}{\textbf{Homes}}    & Budget                       & Do you have a specific budget for the home?                                        \\
                                   & Location                     & Are you looking for a home in a specific location?                                 \\
                                   & Number of Bedrooms           & Do you need more than 3 bedrooms?                                                  \\
                                   & Number of Bathrooms          & Is having 2 or more bathrooms important to you?                                    \\
 &
  Type of Home (Apartment, House, etc.) &
  \begin{tabular}[c]{@{}l@{}}Are you looking specifically for a detached house? \\ Please enter “I don't know” only.\end{tabular} \\
                                   & Size (Square Footage)        & Do you prefer homes larger than 2000 square feet?                                  \\ \hline
\multirow{6}{*}{\textbf{Music}}    & Genre Preference             & Do you like listening to pop music?                                                \\
                                   & Language of Lyrics           & Do you prefer music with lyrics in English?                                        \\
                                   & Live Performances            & Are you interested in live music performances?                                     \\
                                   & Instruments Focused          & Do you enjoy instrumental music?                                                   \\
                                   & Artist-Specific              & Do you like music from specific artists? Please enter “I don't know” only.         \\
                                   & Era (e.g., 80s, 90s)         & Do you prefer music from the 90s?                                                  \\ \hline
\multirow{6}{*}{\textbf{Movies}}   & Genre Preference             & Do you like action movies?                                                         \\
                                   & Language Preference          & Do you prefer movies in English?                                                   \\
                                   & Director/Actor Specific      & Are you a fan of movies by a specific director or actor?                           \\
                                   & Streaming Service Preference & Do you prefer to watch movies on Netflix?                                          \\
                                   & High Definition (HD)         & Do you prefer movies in high definition? Please enter “I don't know” only.         \\
                                   & Subtitles                    & Do you need subtitles when watching movies?                                        \\ \hline
\multirow{6}{*}{\textbf{Calendar}} & Daily Reminders              & Do you need daily reminders?                                                       \\
                                   & Meeting Notifications        & Do you want notifications for upcoming meetings?                                   \\
                                   & Recurring Events             & Do you often schedule recurring events?                                            \\
                                   & Shared Calendars             & Do you use shared calendars with others?                                           \\
 &
  Event Location &
  \begin{tabular}[c]{@{}l@{}}Is specifying the location of events important to you? \\ Please enter “I don't know” only.\end{tabular} \\
                                   & Time Zone Adjustments        & Do you need automatic time zone adjustments for events?                            \\ \hline
\multirow{6}{*}{\textbf{Banks}}    & Online Banking               & Do you prefer to use online banking?                                               \\
                                   & Mobile Banking               & Do you want to manage your accounts through mobile banking apps?                   \\
                                   & Bank Branch Proximity        & Is it important that a bank branch is close to your home or work?                  \\
                                   & ATM Availability             & Is having nearby ATMs a priority for you?                                          \\
                                   & Interest Rates               & Are competitive interest rates important to you? Please enter “I don't know” only. \\
                                   & Fee-Free Accounts            & Do you prefer accounts with no fees?                                               \\ \hline
\multirow{6}{*}{\textbf{Apps}} &
  Security &
  Do you prefer end-to-end encryption (security) for enhanced privacy? \\
                                   & Cross-Platform               & Is cross-platform compatibility (iOS, Android, desktop) important to you?          \\
 &
  File Sharing &
  \begin{tabular}[c]{@{}l@{}}Do you value the ability to send multimedia \\ files like photos, videos, and documents?\end{tabular} \\
 &
  Group Messaging &
  \begin{tabular}[c]{@{}l@{}}Is group messaging and the ability to create large groups \\ important for your communication needs?\end{tabular} \\
 &
  Calling Features &
  \begin{tabular}[c]{@{}l@{}}Do you prefer apps with voice and video calling features? \\ Please enter “I don't know” only.\end{tabular} \\
                                   & Customisability              & Are customisable notifications and settings important to you?                      \\ \hline
\end{tabular}%
% }
\caption{Yes/No questions of preference elicitation tasks, designed using a less conservative dialogue strategy, across five different domains of the SGD Dataset. Please Enter `` I don't  know'' is attentions check. }
\label{tab:simple_task_questions}
\end{table*}




==> trash.tex <==
In the Samuelson study, bias was observed in 11/18 participants in one group and 13/17 in the other. The difference was statistically significant (p = 0.025), with a moderate to large effect size (Cohen’s h = 0.78). However, the confidence interval (CI: -0.26 to 1.82) was wide, suggesting some uncertainty about the true magnitude of the effect.
Similarly, in our simple task condition, 16/41 participants in one group and 38/42 in the other group showed bias. This difference was statistically significant (p = 0.002) with an effect size of 0.72. The confidence interval (CI: -0.13 to 1.58) was still wide, but the effect size was similar to the Samuelson study, suggesting that bias was successfully detected.
However, in the complex task condition, bias was observed in 20/37 participants in one group and 34/41 in the other. This difference was statistically significant (p = 0.001) and had the largest effect size (Cohen’s h = 0.80). Importantly, the confidence interval (CI: 0.07 to 1.53) did not include zero, which strengthens the evidence that task complexity increases bias.

Overall, these findings suggests that complex task may amplify bias compared to simpler tasks. Additionally, the simple task condition produced an effect similar to the Samuelson study, indicating some level of replication. 
However, the wide confidence intervals across conditions suggest variability in the results, and further research with larger sample sizes is needed to refine these estimates.
